Ultrafast quasiparticle dynamics in correlated semimetal Ca$_3$Ru$_2$O$_7$

The correlated polar semimetal Ca$_3$Ru$_2$O$_7$ exhibits a rich phase diagram including two magnetic transitions ($T_N$=56 K and $T_C$=48 K) with the appearance of an insulating-like pseudogap (at $T_C$). In addition, there is a crossover back to metallic behavior at $T^*$=30 K, the origin of which is still under debate. We utilized ultrafast optical pump optical probe spectroscopy to investigate quasiparticle dynamics as a function of temperature in this enigmatic quantum material. We identify two dynamical processes, both of which are influenced by the onset of the pseudogap. This includes electron-phonon relaxation and, below $T_C$, the onset of a phonon bottleneck hindering the relaxation of quasiparticles across the pseudogap. We introduce a gap-modified two-temperature model to describe the temperature dependence of electron-phonon thermalization, and use the Rothwarf-Taylor to model the phonon bottleneck. In conjunction with density functional theory, our experimental results synergistically reveal the origin of the $T$-dependent pseudogap. Further, our data and analysis indicate that $T^*$ emerges as a natural consequence of $T$-dependent gapping out of carriers, and does not correspond to a separate electronic transition. Our results highlight the value of low fluence ultrafast optics as a sensitive probe of low energy electronic structure, thermodynamic parameters, and transport properties of Ruddlesden-Popper ruthenates.

==> Refs <==
@article{Mackenzie1998,
author = {Mackenzie, A P and Haselwimmer, R K W and Tyler, A W and Lonzarich, G G and Mori, Y and Nishizaki, S and Maeno, Y},
file = {:C$\backslash$:/Users/Yakun Yuan/Desktop/PhysRevLett.80.161.pdf:pdf},
journal = {Physical Review Letters},
number = {1},
pages = {161--164},
volume = {80},
title = {{Extremely Strong Dependence of Superconductivity on Disorder in Sr 2 RuO 4}},
year = {1998}
}
@article{Maeno1994,
author = {Maeno, Y and Hashimoto, H and Yoshida, K and Nishizaki, S and Fujita, T and Bednorz, J G and Lichtenberg, F},
file = {:C$\backslash$:/Users/Yakun Yuan/Desktop/372532a0.pdf:pdf},
journal = {Nature},
month = {dec},
pages = {532},
publisher = {Nature Publishing Group},
title = {{Superconductivity in a layered perovskite without copper}},
url = {http://dx.doi.org/10.1038/372532a0 http://10.0.4.14/372532a0},
volume = {372},
year = {1994}
}
@article{Liu1999,
abstract = {We report a Raman-scattering study of the relationship among the charge, spin, and lattice dynamics of Ca3Ru2O7. The metal-insulator (MI) transition (T-MI similar to 48 K) in this compound manifests itself as a rapid suppression of low-frequency electronic scattering intensity, reflecting the opening of a charge gap, Delta(c) similar to 760 cm(-1), and a concomitant softening and broadening of the 438 cm(-1) out-of-phase oxygen phonon mode. Furthermore, the transition to antiferromagnetic order below T-N similar to 56 K is associated with the development of a B-1g resonance peak near 58 cm(-1). We identify this feature as a two-magnon process, based upon which we estimate an in-plane antiferromagnetic exchange coupling of J(parallel to) similar to 8.7 cm(-1) in Ca3Ru2O7. [S0163-1829(99)51334-9].},
author = {Liu, H. L. and Yoon, S. and Cooper, S. L. and Cao, G. and Crow, J. E.},
doi = {10.1103/PhysRevB.60.R6980},
file = {:C$\backslash$:/Users/Yakun Yuan/AppData/Local/Mendeley Ltd/Mendeley Desktop/Downloaded/Liu et al. - 1999 - Raman-scattering study of the charge and spin dynamics of the layered ruthenium oxide Ca3Ru2O7.pdf:pdf},
isbn = {0163-1829},
issn = {0163-1829},
journal = {Physical Review B},
number = {10},
pages = {R6980--R6983},
title = {{Raman-scattering study of the charge and spin dynamics of the layered ruthenium oxide Ca3Ru2O7}},
volume = {60},
year = {1999}
}
@article{Lei2018,
author = {Lei, Shiming and Gu, Mingqiang and Puggioni, Danilo and Stone, Greg and Peng, Jin and Ge, Jianjian and Wang, Yu and Wang, Baoming and Yuan, Yakun and Wang, Ke and Mao, Zhiqiang and Rondinelli, James M. and Gopalan, Venkatraman},
doi = {10.1021/acs.nanolett.8b00633},
file = {:C$\backslash$:/Users/Yakun Yuan/Desktop/acs.nanolett.8b00633.pdf:pdf},
issn = {1530-6984},
journal = {Nano Letters},
keywords = {and stress energies,domain walls,domains,exchange-interaction,ferroelastic switching,in ferroic materials,in situ tem,omain microstructures naturally occur,polar metal,such as electrostatic,to minimize energies related,to their order parameter},
month = {may},
number = {5},
pages = {3088--3095},
title = {{Observation of Quasi-Two-Dimensional Polar Domains and Ferroelastic Switching in a Metal, Ca 3 Ru 2 O 7}},
url = {http://pubs.acs.org/doi/10.1021/acs.nanolett.8b00633},
volume = {18},
year = {2018}
}
@article{Lee2007,
author = {Lee, J. S. and Moon, S. J. and Yang, B. J. and Yu, Jaejun and Schade, U. and Yoshida, Y. and Ikeda, S. I. and Noh, T. W.},
doi = {10.1103/PhysRevLett.98.097403},
file = {:C$\backslash$:/Users/Yakun Yuan/AppData/Local/Mendeley Ltd/Mendeley Desktop/Downloaded/Lee et al. - 2007 - Pseudogap dependence of the optical conductivity spectra of Ca3Ru2O7 A possible contribution of the orbital flip exc.pdf:pdf},
issn = {00319007},
journal = {Physical Review Letters},
number = {9},
pages = {10--13},
title = {{Pseudogap dependence of the optical conductivity spectra of Ca3Ru2O7: A possible contribution of the orbital flip excitation}},
volume = {98},
year = {2007}
}
@article{Yoshida2004,
author = {Yoshida, Yoshiyuki and Nagai, Ichiro and Ikeda, Shin-Ichi and Shirakawa, Naoki and Kosaka, Masashi and M{\^{o}}ri, Nobuo},
file = {:C$\backslash$:/Users/Yakun Yuan/AppData/Local/Mendeley Ltd/Mendeley Desktop/Downloaded/Yoshida et al. - 2004 - Quasi-two-dimensional metallic ground state of Ca3Ru2O7.pdf:pdf},
journal = {Physical Review B},
pages = {220411(R)},
title = {{Quasi-two-dimensional metallic ground state of Ca3Ru2O7}},
volume = {69},
year = {2004}
}
@article{Cao1997,
abstract = {Single crystal Ca3Ru2O7 shows a metallic antiferromagnetic phase intermediate between a first-order metal to nonmetal transition at TM = 48K and the antiferromagnetic ordering (N{\'{e}}el) temperature, TN = 56K. The metallic antiferromagnetic phase is predicted within various Mott-Hubbard models. Magnetization and electrical resistivity reveal strongly anisotropic metamagnetism in the nonmetallic antiferromagnetic phase. The charge and spin excitations are strongly coupled: The H-T phase diagrams determined by magnetization and magnetoresistivity are indistinguishable and reveal a multicritical point. The heat capacity of Ca3Ru2O7 suggests it is a highly correlated electron system.},
author = {Cao, G. and McCall, S. and Crow, J. and Guertin, R.},
doi = {10.1103/PhysRevLett.78.1751},
file = {:C$\backslash$:/Users/Yakun Yuan/AppData/Local/Mendeley Ltd/Mendeley Desktop/Downloaded/Cao et al. - 1997 - Observation of a Metallic Antiferromagnetic Phase and Metal to Nonmetal Transition in Ca3Ru2O7.pdf:pdf},
issn = {0031-9007},
journal = {Physical Review Letters},
number = {9},
pages = {1751--1754},
title = {{Observation of a Metallic Antiferromagnetic Phase and Metal to Nonmetal Transition in Ca3Ru2O7}},
volume = {78},
year = {1997}
}
@article{Cao2004,
  author={G Cao and X N Lin and L Balicas and S Chikara and J E Crow and P Schlottmann},
  title={Orbitally driven behaviour: Mott transition, quantum oscillations and colossal magnetoresistance in bilayered Ca 3 Ru 2 O 7},
  journal={New Journal of Physics},
  volume={6},
  number={1},
  pages={159},
  url={http://stacks.iop.org/1367-2630/6/i=1/a=159},
  year={2004},
  abstract={We report recent transport and thermodynamic experiments over a wide range of temperatures for the Mott-like system Ca 3 Ru 2 O 7 at high magnetic fields, B (â‰¤ 30 T). This work reveals a rich and highly anisotropic phase diagram, where applying B along the a -, b -, and c -axis leads to vastly different behaviour. A fully spin-polarized state via a first-order metamagnetic transition is obtained for B â‰¥ 6 T and B || a , and colossal magnetoresistance is seen for B || b , and quantum oscillations in the resistivity are observed for B || c , respectively. The interplay of the lattice, orbital and spin degrees of freedom are believed to give rise to this strongly anisotropic behaviour.}
}
@article{Peng2013,
author = {Peng, Jin and Ke, X. and Wang, Gaochao and Ortmann, J. E. and Fobes, David and Hong, Tao and Tian, Wei and Wu, Xiaoshan and Mao, Z. Q.},
doi = {10.1103/PhysRevB.87.085125},
file = {:C$\backslash$:/Users/Yakun Yuan/AppData/Local/Mendeley Ltd/Mendeley Desktop/Downloaded/Peng et al. - 2013 - From quasi-two-dimensional metal with ferromagnetic bilayers to Mott insulator with G-type antiferromagnetic order.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {8},
pages = {1--7},
title = {{From quasi-two-dimensional metal with ferromagnetic bilayers to Mott insulator with G-type antiferromagnetic order in Ca3(Ru 1-xTix)2O7}},
volume = {87},
year = {2013}
}

@article{Baumberger2006,
  title = {Nested Fermi Surface and Electronic Instability in ${\mathrm{Ca}}_{3}{\mathrm{Ru}}_{2}{\mathrm{O}}_{7}$},
  author = {Baumberger, F. and Ingle, N. J. C. and Kikugawa, N. and Hossain, M. A. and Meevasana, W. and Perry, R. S. and Shen, K. M. and Lu, D. H. and Damascelli, A. and Rost, A. and Mackenzie, A. P. and Hussain, Z. and Shen, Z.-X.},
  journal = {Phys. Rev. Lett.},
  volume = {96},
  issue = {10},
  pages = {107601},
  numpages = {4},
  year = {2006},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.96.107601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.96.107601}
}

@article{Kikugawa2010,
author = {Kikugawa ,Naoki and Winfried Rost ,Andreas and William Hicks ,Clifford and John Schofield ,Andrew and Peter Mackenzie ,Andrew},
title = {Ca3Ru2O7: Density Wave Formation and Quantum Oscillations in the Hall Resistivity},
journal = {Journal of the Physical Society of Japan},
volume = {79},
number = {2},
pages = {024704},
year = {2010},
doi = {10.1143/JPSJ.79.024704},
URL = {https://doi.org/10.1143/JPSJ.79.024704},
eprint = {https://doi.org/10.1143/JPSJ.79.024704}
}

@article{Xing2018,
  title = {Existence of electron and hole pockets and partial gap opening in the correlated semimetal ${\mathbf{Ca}}_{\mathbf{3}}{\mathbf{Ru}}_{\mathbf{2}}{\mathbf{O}}_{\mathbf{7}}$},
  author = {Xing, Hui and Wen, Libin and Shen, Chenyi and He, Jiaming and Cai, Xinxin and Peng, Jin and Wang, Shun and Tian, Mingliang and Xu, Zhu-An and Ku, Wei and Mao, Zhiqiang and Liu, Ying},
  journal = {Phys. Rev. B},
  volume = {97},
  issue = {4},
  pages = {041113},
  numpages = {5},
  year = {2018},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.97.041113},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.97.041113}
}

@article{Kabanov1999,
  title = {Quasiparticle relaxation dynamics in superconductors with different gap structures: Theory and experiments on ${\mathrm{YBa}}_{2}{\mathrm{Cu}}_{3}{\mathrm{O}}_{7\mathrm{\ensuremath{-}}\mathrm{\ensuremath{\delta}}}$},
  author = {Kabanov, V. V. and Demsar, J. and Podobnik, B. and Mihailovic, D.},
  journal = {Phys. Rev. B},
  volume = {59},
  issue = {2},
  pages = {1497--1506},
  numpages = {0},
  year = {1999},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.59.1497},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.59.1497}
}

@article{Demsar1999,
  title = {Single Particle and Collective Excitations in the One-Dimensional Charge Density Wave Solid ${\mathrm{K}}_{0.3}{\mathrm{MoO}}_{3}$ Probed in Real Time by Femtosecond Spectroscopy},
  author = {Demsar, J. and Biljakovi\ifmmode \acute{c}\else \'{c}\fi{}, K. and Mihailovic, D.},
  journal = {Phys. Rev. Lett.},
  volume = {83},
  issue = {4},
  pages = {800--803},
  numpages = {0},
  year = {1999},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.83.800},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.83.800}
}

@article{Demsar2003,
  title = {Pair-Breaking and Superconducting State Recovery Dynamics in ${\mathrm{M}\mathrm{g}\mathrm{B}}_{2}$},
  author = {Demsar, J. and Averitt, R. D. and Taylor, A. J. and Kabanov, V. V. and Kang, W. N. and Kim, H. J. and Choi, E. M. and Lee, S. I.},
  journal = {Phys. Rev. Lett.},
  volume = {91},
  issue = {26},
  pages = {267002},
  numpages = {4},
  year = {2003},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.91.267002},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.91.267002}
}

@article{Demsar2006,
  author={Jure Demsar and John L Sarrao and Antoinette J Taylor},
  title={Dynamics of photoexcited quasiparticles in heavy electron compounds},
  journal={Journal of Physics: Condensed Matter},
  volume={18},
  number={16},
  pages={R281},
  url={http://stacks.iop.org/0953-8984/18/i=16/a=R01},
  year={2006},
  abstract={Femtosecond real-time spectroscopy is an emerging new tool for studying low energy electronic structure in correlated electron systems. Motivated by recent advances in understanding the nature of relaxation phenomena in various correlated electron systems (superconductors, density wave systems) the technique has been applied to heavy electron compounds in comparison with their non-magnetic counterparts. While the dynamics in their non-magnetic analogues are similar to the dynamics observed in noble metals (only weak temperature dependences are observed) and can be treated with a simple two-temperature model, the photoexcited carrier dynamics in heavy electron systems show dramatic changes as a function of temperature and excitation level. In particular, below some characteristic temperature the relaxation rate starts to decrease, dropping by more than two orders of magnitude upon cooling down to liquid He temperatures. This behaviour has been consistently observed in various heavy fermion metals as well as Kondo insulators, and is believed to be quite general. In order to account for the experimental observations, two theoretical models have been proposed. The first treats the heavy electron systems as simple metals with very flat electron dispersion near the Fermi level. An electron‚Äìphonon thermalization scenario can account for the observed slowing down of the relaxation provided that there exists a mechanism for suppression of electron‚Äìphonon scattering when both the initial and final electronic states lie in the region of flat dispersion. An alternative scenario argues that the relaxation dynamics in heavy electron systems are governed by the Rothwarf‚ÄìTaylor bottleneck, where the dynamics are governed by the presence of a narrow gap in the density of states near the Fermi level. The so-called hybridization gap results from hybridization between localized moments and the conduction electron background. Remarkable agreement with the model suggests that carrier relaxation in a broad class of heavy electron systems (both metals and insulators) is governed by the presence of a (weakly temperature dependent) indirect hybridization gap. Here we review the experimental results on a variety of heavy electron compounds, point out the common features as well as the peculiarities observed in some compounds, and compare the data with existing theoretical models.}
}

@article{Rothwarf1967,
  title = {Measurement of Recombination Lifetimes in Superconductors},
  author = {Rothwarf, Allen and Taylor, B. N.},
  journal = {Phys. Rev. Lett.},
  volume = {19},
  issue = {1},
  pages = {27--30},
  numpages = {0},
  year = {1967},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.19.27},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.19.27}
}

@article{Demsar2001,
  title = {Quasiparticle dynamics and gap structure in $\mathrm{Hg}{\mathrm{Ba}}_{2}{\mathrm{Ca}}_{2}{\mathrm{Cu}}_{3}{\mathrm{O}}_{8+\ensuremath{\delta}}$ investigated with femtosecond spectroscopy},
  author = {Demsar, J. and Hudej, R. and Karpinski, J. and Kabanov, V. V. and Mihailovic, D.},
  journal = {Phys. Rev. B},
  volume = {63},
  issue = {5},
  pages = {054519},
  numpages = {7},
  year = {2001},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.63.054519},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.63.054519}
}

@article{Gedik2004,
  title = {Single-quasiparticle stability and quasiparticle-pair decay in ${\mathrm{YBa}}_{2}{\mathrm{Cu}}_{3}{\mathrm{O}}_{6.5}$},
  author = {Gedik, N. and Blake, P. and Spitzer, R. C. and Orenstein, J. and Liang, Ruixing and Bonn, D. A. and Hardy, W. N.},
  journal = {Phys. Rev. B},
  volume = {70},
  issue = {1},
  pages = {014504},
  numpages = {13},
  year = {2004},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.70.014504},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.70.014504}
}

@article{Kabanov2005,
  title = {Kinetics of a Superconductor Excited with a Femtosecond Optical Pulse},
  author = {Kabanov, V. V. and Demsar, J. and Mihailovic, D.},
  journal = {Phys. Rev. Lett.},
  volume = {95},
  issue = {14},
  pages = {147002},
  numpages = {4},
  year = {2005},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.95.147002},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.95.147002}
}

@article{Torchinsky2010,
  title = {Band-dependent Quasiparticle Dynamics in Single Crystals of the ${\mathrm{Ba}}_{0.6}{\mathbf{K}}_{0.4}{\mathrm{Fe}}_{2}{\mathrm{As}}_{2}$ Superconductor Revealed by Pump-Probe Spectroscopy},
  author = {Torchinsky, Darius H. and Chen, G. F. and Luo, J. L. and Wang, N. L. and Gedik, Nuh},
  journal = {Phys. Rev. Lett.},
  volume = {105},
  issue = {2},
  pages = {027005},
  numpages = {4},
  year = {2010},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.105.027005},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.105.027005}
}
@article{Ke2014,
  title = {Commensurate-incommensurate magnetic phase transition in the Fe-doped bilayer ruthenate ${\mathrm{Ca}}_{3}{\mathrm{Ru}}_{2}{\mathrm{O}}_{7}$},
  author = {Ke, X. and Peng, J. and Tian, W. and Hong, Tao and Zhu, M. and Mao, Z. Q.},
  journal = {Phys. Rev. B},
  volume = {89},
  issue = {22},
  pages = {220407},
  numpages = {5},
  year = {2014},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.89.220407},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.89.220407}
}
@article{Chia2006,
abstract = {Ultrafast time-resolved photoinduced reflectivity is measured for the itinerant antiferromagnet UNiGa{\$}{\_}{\{}5{\}}{\$} ({\$}T{\_}{\{}N{\}} \backslashapprox{\$}85 K) from room temperature to 10 K. The relaxation time {\$}\backslashtau{\$} shows a sharp increase at {\$}T{\_}{\{}N{\}}{\$} consistent with the opening of a spin gap. In addition, the temperature dependence of {\$}\backslashtau{\$} below {\$}T{\_}{\{}N{\}}{\$} is consistent with the opening of a spin gap leading to a quasiparticle recombination bottleneck as revealed by the Rothwarf-Taylor model. This contrasts with canonical heavy fermions such as CeCoIn{\$}{\_}{\{}5{\}}{\$} where the recombination bottleneck arises from the hybridization gap.},
archivePrefix = {arXiv},
arxivId = {cond-mat/0605240},
author = {Chia, Elbert E.M. and Zhu, Jian Xin and Lee, H J and Hur, Namjung and Moreno, N O and Bauer, E D and Durakiewicz, T and Averitt, R D and Sarrao, J L and Taylor, A J},
doi = {10.1103/PhysRevB.74.140409},
eprint = {0605240},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/Chia et al. - 2006 - Quasiparticle relaxation across the spin-density-wave gap in the itinerant antiferromagnet UNi Ga5.pdf:pdf},
issn = {10980121},
journal = {Physical Review B - Condensed Matter and Materials Physics},
number = {14},
pages = {5--8},
primaryClass = {cond-mat},
title = {{Quasiparticle relaxation across the spin-density-wave gap in the itinerant antiferromagnet UNi Ga5}},
volume = {74},
year = {2006}
}
@article{Groeneveld1995,
abstract = {},
author = {Groeneveld, Rogier H. M. and Sprik, R. and Lagendijk, Ad},
doi = {10.1103/PhysRevB.51.11433},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/PhysRevB.51.11433.pdf:pdf},
isbn = {0163-1829},
issn = {0163-1829},
journal = {Phys. Rev. B},
number = {17},
pages = {11433},
pmid = {9977873},
title = {{Femtosecond spectroscopy of electron-electron and alectron-phonon energy relaxation in Ag aund Au}},
volume = {51},
year = {1995}
}
@article{Schmidt2008,
abstract = {},
author = {Schmidt, Aaron J. and Chen, Xiaoyuan and Chen, Gang},
doi = {10.1063/1.3006335},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/Schmidt, Chen, Chen - 2008 - Pulse accumulation, radial heat conduction, and anisotropic thermal conductivity in pump-probe transient(2).pdf:pdf},
isbn = {0034-6748},
issn = {00346748},
journal = {Review of Scientific Instruments},
number = {11},
pmid = {19045906},
title = {{Pulse accumulation, radial heat conduction, and anisotropic thermal conductivity in pump-probe transient thermoreflectance}},
volume = {79},
year = {2008}
}
@article{Schmidt20082,
author = {Schmidt, Aaron J.},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/Schmidt - 2008 - Optical characterization of thermal transport from the nanoscale to the macroscale(2).pdf:pdf},
journal = {Dissertation},
title = {{Optical characterization of thermal transport from the nanoscale to the macroscale}},
url = {http://dspace.mit.edu/handle/1721.1/44798},
year = {2008}
}
@article{Sup,
author = {},
file = {},
journal = {Supplementary Materials},
title = {{Supplementary Materials: Quasiparticle relaxation across pseudogap in polar metal Ca$_3$Ru$_2$O$_7$}},
url = {},
year = {2008}
}
@article{Chia2007,
abstract = {},
author = {Chia, Elbert E M and Zhu, Jian Xin and Talbayev, D and Averitt, R D and Taylor, A J and Oh, Kyu Hwan and Jo, In Sun and Lee, S. I.},
doi = {10.1103/PhysRevLett.99.147008},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/Chia et al. - 2007 - Observation of competing order in a high-Tc superconductor using femtosecond optical pulses.pdf:pdf},
isbn = {0031-9007},
issn = {00319007},
journal = {Physical Review Letters},
number = {14},
pages = {1--4},
title = {{Observation of competing order in a high-Tc superconductor using femtosecond optical pulses}},
volume = {99},
year = {2007}
}
@article{MacDonald2000,
author = {MacDonald, A H and Fisher, Matthew P A},
doi = {10.1103/PhysRevB.61.5724},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/PhysRevB.61.5724.pdf:pdf},
issn = {0163-1829},
journal = {Physical Review B},
month = {feb},
number = {8},
pages = {5724--5733},
title = {{Quantum theory of quantum Hall smectics}},
url = {http://link.aps.org/doi/10.1103/PhysRevB.61.5724 https://link.aps.org/doi/10.1103/PhysRevB.61.5724},
volume = {61},
year = {2000}
}
@article{Pack1977,
abstract = {A method is given for generating sets of special points in the Brillouin zone which provides an efficient means of integrating periodic functions of the wave vector. The integration can be over the entire Brillouin zone or over specified portions thereof. This method also has applications in spectral and density-of-state calculations. The relationships to the Chadi-Cohen and Gilat-Raubenheimer methods are indicated.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Pack, James D. and Monkhorst, Hendrik J.},
doi = {10.1103/PhysRevB.16.1748},
eprint = {arXiv:1011.1669v3},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/PhysRevB.13.5188.pdf:pdf},
isbn = {0556-2805},
issn = {0556-2805},
journal = {Physical Review B},
month = {aug},
number = {4},
pages = {1748--1749},
pmid = {1966486},
title = {{"Special points for Brillouin-zone integrations"â€”a reply}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.16.1748},
volume = {16},
year = {1977}
}
@article{Kresse1999,
abstract = {},
archivePrefix = {arXiv},
arxivId = {10.1016/0927-0256(96)00008},
author = {Kresse, G. and Joubert, D.},
doi = {10.1103/PhysRevB.59.1758},
eprint = {0927-0256(96)00008},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/PhysRevB.59.1758.pdf:pdf},
isbn = {0163-1829},
issn = {0163-1829},
journal = {Physical Review B},
month = {jan},
number = {3},
pages = {1758--1775},
pmid = {19309091},
primaryClass = {10.1016},
title = {{From ultrasoft pseudopotentials to the projector augmented-wave method}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.59.1758},
volume = {59},
year = {1999}
}
@article{Perdew2008,
abstract = {},
archivePrefix = {arXiv},
arxivId = {0707.2088},
author = {Perdew, John P. and Ruzsinszky, Adrienn and Csonka, G{\'{a}}bor I. and Vydrov, Oleg A. and Scuseria, Gustavo E. and Constantin, Lucian A. and Zhou, Xiaolan and Burke, Kieron},
doi = {10.1103/PhysRevLett.100.136406},
eprint = {0707.2088},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/PhysRevLett.100.136406.pdf:pdf},
isbn = {0031-9007},
issn = {0031-9007},
journal = {Physical Review Letters},
month = {apr},
number = {13},
pages = {136406},
pmid = {18517979},
title = {{Restoring the Density-Gradient Expansion for Exchange in Solids and Surfaces}},
url = {http://arxiv.org/abs/0707.2088{\%}0Ahttp://dx.doi.org/10.1103/PhysRevLett.100.136406 https://link.aps.org/doi/10.1103/PhysRevLett.100.136406},
volume = {100},
year = {2008}
}
@article{Blochl1994,
abstract = {},
archivePrefix = {arXiv},
arxivId = {arXiv:1408.4701v2},
author = {Bl{\"{o}}chl, P. E.},
doi = {10.1103/PhysRevB.50.17953},
eprint = {arXiv:1408.4701v2},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/Bl{\"{o}}chl - 1994 - Projector augmented-wave method(2).pdf:pdf},
isbn = {0163-1829 (Print)$\backslash$n0163-1829 (Linking)},
issn = {0163-1829},
journal = {Physical Review B},
month = {dec},
number = {24},
pages = {17953--17979},
pmid = {9976227},
title = {{Projector augmented-wave method}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.50.17953},
volume = {50},
year = {1994}
}
@article{Kresse1996,
abstract = {},
archivePrefix = {arXiv},
arxivId = {10.1016/0927-0256(96)00008},
author = {Kresse, G. and Furthm{\"{u}}ller, J.},
doi = {10.1103/PhysRevB.54.11169},
eprint = {0927-0256(96)00008},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/Kresse, Furthm{\"{u}}ller - 1996 - Efficient iterative schemes for iab initioi total-energy calculations using a plane-wave basis set(2).pdf:pdf},
isbn = {1098-0121},
issn = {0163-1829},
journal = {Physical Review B},
month = {oct},
number = {16},
pages = {11169--11186},
pmid = {9984901},
primaryClass = {10.1016},
title = {{Efficient iterative schemes for ab initio total-energy calculations using a plane-wave basis set}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.54.11169},
volume = {54},
year = {1996}
}

@article{Yoshida2005,
abstract = {.},
archivePrefix = {arXiv},
arxivId = {cond-mat/0412386},
author = {Yoshida, Yoshiyuki and Ikeda, Shin-Ichi and Matsuhata, Hirofumi and Shirakawa, Naoki and Lee, C. H. and Katano, Susumu},
doi = {10.1103/PhysRevB.72.054412},
eprint = {0412386},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/Yoshida et al. - 2005 - Crystal and magnetic structure of math display=inline mrow msub mi mathvariant=normalCami mn3mn msub msub mi (2).pdf:pdf},
issn = {1098-0121},
journal = {Physical Review B},
number = {5},
pages = {054412},
primaryClass = {cond-mat},
title = {{Crystal and magnetic structure of {\textless}math display="inline"{\textgreater} {\textless}mrow{\textgreater} {\textless}msub{\textgreater} {\textless}mi mathvariant="normal"{\textgreater}Ca{\textless}/mi{\textgreater} {\textless}mn{\textgreater}3{\textless}/mn{\textgreater} {\textless}/msub{\textgreater} {\textless}msub{\textgreater} {\textless}mi mathvariant="normal"{\textgreater}Ru{\textless}/mi{\textgreater} {\textless}mn{\textgreater}2{\textless}/mn{\textgreater} {\textless}/msub{\textgreater} {\textless}msub{\textgreater} {\textless}mi mathvariant="normal"{\textgreater}O{\textless}/mi{\textgreater} {\textless}mn{\textgreater}7{\textless}/mn{\textgreater} {\textless}/msub{\textgreater} {\textless}/mrow{\textgreater} {\textless}/math}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.72.054412 http://link.aps.org/doi/10.1103/PhysRevB.72.054412},
volume = {72},
year = {2005}
}

@article{Ghosh2017,
abstract = {},
author = {Ghosh, Tufan and Aharon, Sigalit and Etgar, Lioz and Ruhman, Sanford},
doi = {10.1021/jacs.7b09508},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/jacs.7b09508.pdf:pdf},
isbn = {1520-5126 (Electronic) 0002-7863 (Linking)},
issn = {15205126},
journal = {Journal of the American Chemical Society},
number = {50},
pages = {18262--18270},
pmid = {29172490},
title = {{Free Carrier Emergence and Onset of Electron-Phonon Coupling in Methylammonium Lead Halide Perovskite Films}},
volume = {139},
year = {2017}
}
@article{Batignani2018,
abstract = {},
archivePrefix = {arXiv},
arxivId = {1705.08687},
author = {Batignani, Giovanni and Fumero, Giuseppe and {Srimath Kandada}, Ajay Ram and Cerullo, Giulio and Gandini, Marina and Ferrante, Carino and Petrozza, Annamaria and Scopigno, Tullio},
doi = {10.1038/s41467-018-04367-6},
eprint = {1705.08687},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/s41467-018-04367-6.pdf:pdf},
issn = {20411723},
journal = {Nature Communications},
number = {1},
pages = {1--5},
publisher = {Springer US},
title = {{Probing femtosecond lattice displacement upon photo-carrier generation in lead halide perovskite}},
url = {http://dx.doi.org/10.1038/s41467-018-04367-6},
volume = {9},
year = {2018}
}
@article{Park2018,
abstract = {},
author = {Park, Myeongkee and Neukirch, Amanda J. and Reyes-Lillo, Sebastian E. and Lai, Minliang and Ellis, Scott R. and Dietze, Daniel and Neaton, Jeffrey B. and Yang, Peidong and Tretiak, Sergei and Mathies, Richard A.},
doi = {10.1038/s41467-018-04946-7},
file = {:D$\backslash$:/OneDrive - The Pennsylvania State University/Mendeley Desktop/s41467-018-04946-7.pdf:pdf},
isbn = {4146701804946},
issn = {20411723},
journal = {Nature Communications},
number = {1},
pages = {1--9},
publisher = {Springer US},
title = {{Excited-state vibrational dynamics toward the polaron in methylammonium lead iodide perovskite}},
url = {http://dx.doi.org/10.1038/s41467-018-04946-7},
volume = {9},
year = {2018}
}

